Context-Aware Transfer Attacks for Object Detection

Blackbox transfer attacks for image classifiers have been extensively studied in recent years. In contrast, little progress has been made on transfer attacks for object detectors. Object detectors take a holistic view of the image and the detection of one object (or lack thereof) often depends on other objects in the scene. This makes such detectors inherently context-aware and adversarial attacks in this space are more challenging than those targeting image classifiers. In this paper, we present a new approach to generate context-aware attacks for object detectors. We show that by using co-occurrence of objects and their relative locations and sizes as context information, we can successfully generate targeted mis-categorization attacks that achieve higher transfer success rates on blackbox object detectors than the state-of-the-art. We test our approach on a variety of object detectors with images from PASCAL VOC and MS COCO datasets and demonstrate up to $20$ percentage points improvement in performance compared to the other state-of-the-art methods.

==> AAAI2022/figs/fig-visualization-spp.tex <==
% \begin{figure*}[!ht]
% \centering 
% \hspace*{-1cm} 
% \includegraphics[scale=0.75]{AAAI2022/figs/visualization.pdf}
% \caption{
% }
% \label{fig:visualization}
% \end{figure*}

\begin{figure*}[!ht]
    \centering 
    \begin{subfigure}[t]{0.9\linewidth}
    \includegraphics[width=1\linewidth]{AAAI2022/figs/visualization-voc-eps20_.pdf}
    \caption{PASCAL VOC, $L_{\infty} \le 20$}
    \end{subfigure}
    \begin{subfigure}[t]{0.75\linewidth}
    \includegraphics[width=1\textwidth]{AAAI2022/figs/visualization-voc-eps30.pdf}
    \caption{PASCAL VOC, $L_{\infty} \le 30$}
    \end{subfigure}
    % \par\bigskip
    \begin{subfigure}[t]{0.75\linewidth}
    \includegraphics[width=1\linewidth]{AAAI2022/figs/visualization-coco-eps10.pdf}
    \caption{MS COCO, $L_{\infty} \le 10$}
    \end{subfigure}
    \begin{subfigure}[t]{0.75\linewidth}
    \includegraphics[width=1\textwidth]{AAAI2022/figs/visualization-coco-eps20.pdf}
    \caption{MS COCO, $L_{\infty} \le 20$}
    \end{subfigure}
    \begin{subfigure}[t]{0.75\linewidth}
    \includegraphics[width=1\textwidth]{AAAI2022/figs/visualization-coco-eps30.pdf}
    \caption{MS COCO, $L_{\infty} \le 30$}
    \end{subfigure}
    \caption{We visualize three examples where baseline attack fails but our context-aware method succeeds by introducing helper objects in the attack. The perturbation ($L_{\infty} \le 10$) is generated from our perturbation machine (whitebox ensemble of FRCNN and YOLOv3) and tested on the blackbox model (RetinaNet). The detection results on original image, image perturbed by baseline attack, and image perturbed by our context-aware method are shown in the subfigures from left to right. In these examples, we introduce pottedplant as a helper object to mis-categorize the victim monitor to sofa, introduce another bird to mis-categorize the person to a bird, and add a few chairs to mis-categorize the cow to a sofa. Visualization of perturbation level $L_{\infty} <= 20, 30$ can be found in supplementary materials.}
    \label{fig:visualization_supp}
\end{figure*}

==> AAAI2022/tables/tab-coco.tex <==
\begin{table*}[]
\centering
\caption{White-box and black-box attack performance on different models with different perturbation budgets using MS COCO dataset.}
\label{tab:coco}
\begin{tabular}{cccc|cccccc}
\hline
\multirow{2}{*}{Perturbation Budget} & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{\textbf{Whitebox}} & \multicolumn{6}{c}{\textbf{Blackbox}} \\ \cline{3-10} 
                                   &          & FRCNN & YOLOv3 & Retina & Libra & Fovea & Free & DETR & D-DETR \\ \hline
\multirow{3}{*}{$L_{\infty} = 5$}  & Baseline & 11.2  & 14.4  & 3.2    & 1.2   & 4.8   & 7.6  & 2.2  & 7.0    \\
                                   & Ours     & 17.6  & 27.6  & 5.0    & 3.0   & 8.4   & 12.0 & 4.6  & 14.6   \\
                                   & Random   & 16.2  & 23.6  & 4.8    & 2.4   & 8.0   & 10.4 & 4.2  & 12.2   \\ \hline
\multirow{3}{*}{$L_{\infty} = 10$} & Baseline & 29.0  & 32.2  & 7.4    & 4.8   & 11.6  & 16.6 & 3.4  & 19.0   \\
                                   & Ours     & 41.2  & 54.4  & 12.0   & 11.2  & 18.6  & 25.0 & 10.8 & 27.8   \\
                                   & Random   & 40.2  & 48.4  & 11.2   & 8.0   & 14.6  & 20.0 & 6.2  & 23.6   \\ \hline
\multirow{3}{*}{$L_{\infty} = 20$} & Baseline & 51.8  & 49.2  & 13.4   & 11.8  & 22.0  & 28.6 & 8.8  & 26.8   \\
                                   & Ours     & 64.4  & 70.0  & 20.8   & 22.2  & 35.4  & 40.8 & 20.0 & 43.2   \\
                                   & Random   & 60.6  & 66.4  & 20.6   & 18.8  & 31.4  & 37.2 & 20.2 & 39.2   \\ \hline
\multirow{3}{*}{$L_{\infty} = 30$} & Baseline & 57.6  & 54.4  & 18.2   & 15.4  & 25.6  & 34.8 & 8.0  & 28.8   \\
                                   & Ours     & 68.6  & 75.4  & 27.2   & 27.2  & 39.2  & 46.2 & 21.2 & 48.6   \\
                                   & Random   & 65.8  & 73.6  & 23.8   & 21.8  & 34.8  & 47.8 & 18.4 & 42.0   \\ \hline
\multirow{3}{*}{$L_{\infty} = 40$} & Baseline & 58.2  & 56.2  & 19.4   & 14.8  & 29.8  & 37.2 & 11.8 & 29.8   \\
                                   & Ours     & 70.8  & 77.8  & 28.8   & 30.4  & 42.4  & 49.4 & 25.6 & 46.8   \\
                                   & Random   & 67.2  & 73.0  & 26.6   & 24.2  & 38.2  & 47.8 & 22.6 & 43.4   \\ \hline
\end{tabular}
\end{table*}

==> AAAI2022/tables/tab-combined-all.tex <==
\begin{table*}[]
\centering
\caption{White-box and black-box attack fooling rate on different models with different perturbation budgets using PASCAL VOC and MS COCO dataset.\Salnote{This table is taking too much space. Maybe we can use $L_\infty =  10, 20, 30$ in the main paper, and move the full table to supplementary. Also, we should add some colors to baseline/ours/random to make it easy for readers to understand. Maybe move Ours to third rows?} }
\label{tab:combined}
\begin{tabular}{cccc|cccccc}
% \hline
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Perturbation \\ Budget\end{tabular}} &
  \multirow{2}{*}{Method} &
  \multicolumn{2}{c|}{\textbf{Whitebox}} &
  \multicolumn{6}{c}{\textbf{Blackbox}} \\ 
%   \cline{3-10} 
                                   &          & FRCNN & YOLOv3 & Retina & Libra & Fovea & Free & DETR & D-DETR \\ \hline

\addlinespace
\multicolumn{10}{c}{\textbf{\textit{Results on PASCAL VOC}}}\\
\multirow{3}{*}{$L_{\infty} = 5$}  & Baseline & 13.2  & 29.2   & 4.8    & 4.2   & 8.0   & 13.4 & 5.0  & 12.2   \\
                                   & Ours     & 24.8  & 50.0   & 8.8    & 9.0   & 16.6  & 21.4 & 11.2 & 25.6   \\
                                   & Random   & 20.0  & 46.2   & 8.4    & 7.4   & 15.0  & 20.0 & 8.8  & 20.2   \\ \hline
\multirow{3}{*}{$L_{\infty} = 10$} & Baseline & 40.0  & 53.8   & 13.8   & 9.2   & 22.2  & 27.4 & 9.6  & 23.2   \\
                                   & Ours     & 55.8  & 75.6   & 22.6   & 20.4  & 33.6  & 39.2 & 20.2 & 39.2   \\
                                   & Random   & 52.4  & 69.2   & 19.4   & 17.4  & 31.6  & 37.8 & 17.4 & 36.8   \\ \hline
\multirow{3}{*}{$L_{\infty} = 20$} & Baseline & 65.2  & 67.8   & 24.0   & 21.4  & 34.4  & 41.8 & 14.4 & 37.6   \\
                                   & Ours     & 78.6  & 87.2   & 35.2   & 38.4  & 51.6  & 56.6 & 34.0 & 58.4   \\
                                   & Random   & 74.4  & 83.8   & 31.0   & 29.6  & 46.2  & 54.4 & 28.0 & 52.6   \\ \hline
\multirow{3}{*}{$L_{\infty} = 30$} & Baseline & 70.6  & 70.4   & 29.8   & 28.6  & 41.6  & 48.0 & 20.4 & 38.6   \\
                                   & Ours     & 80.6  & 88.0   & 42.0   & 44.2  & 56.8  & 63.6 & 40.2 & 59.0   \\
                                   & Random   & 79.2  & 82.6   & 37.8   & 36.8  & 53.4  & 59.8 & 34.4 & 52.8   \\ \hline
\multirow{3}{*}{$L_{\infty} = 40$} & Baseline & 73.4  & 73.2   & 30.8   & 27.0  & 41.8  & 47.6 & 21.6 & 41.2   \\
                                   & Ours     & 85.4  & 90.2   & 43.6   & 45.2  & 60.2  & 63.4 & 41.8 & 62.4   \\
                                   & Random   & 82.2  & 85.4   & 40.0   & 38.8  & 54.0  & 62.2 & 37.0 & 57.4   \\ \hline

\addlinespace
\multicolumn{10}{c}{\textbf{\textit{Results on MS COCO}}}\\
\multirow{3}{*}{$L_{\infty} = 5$}  & Baseline & 11.2  & 14.4  & 3.2    & 1.2   & 4.8   & 7.6  & 2.2  & 7.0    \\
                                   & Ours     & 17.6  & 27.6  & 5.0    & 3.0   & 8.4   & 12.0 & 4.6  & 14.6   \\
                                   & Random   & 16.2  & 23.6  & 4.8    & 2.4   & 8.0   & 10.4 & 4.2  & 12.2   \\ \hline
\multirow{3}{*}{$L_{\infty} = 10$} & Baseline & 29.0  & 32.2  & 7.4    & 4.8   & 11.6  & 16.6 & 3.4  & 19.0   \\
                                   & Ours     & 41.2  & 54.4  & 12.0   & 11.2  & 18.6  & 25.0 & 10.8 & 27.8   \\
                                   & Random   & 40.2  & 48.4  & 11.2   & 8.0   & 14.6  & 20.0 & 6.2  & 23.6   \\ \hline
\multirow{3}{*}{$L_{\infty} = 20$} & Baseline & 51.8  & 49.2  & 13.4   & 11.8  & 22.0  & 28.6 & 8.8  & 26.8   \\
                                   & Ours     & 64.4  & 70.0  & 20.8   & 22.2  & 35.4  & 40.8 & 20.0 & 43.2   \\
                                   & Random   & 60.6  & 66.4  & 20.6   & 18.8  & 31.4  & 37.2 & 20.2 & 39.2   \\ \hline
\multirow{3}{*}{$L_{\infty} = 30$} & Baseline & 57.6  & 54.4  & 18.2   & 15.4  & 25.6  & 34.8 & 8.0  & 28.8   \\
                                   & Ours     & 68.6  & 75.4  & 27.2   & 27.2  & 39.2  & 46.2 & 21.2 & 48.6   \\
                                   & Random   & 65.8  & 73.6  & 23.8   & 21.8  & 34.8  & 47.8 & 18.4 & 42.0   \\ \hline
\multirow{3}{*}{$L_{\infty} = 40$} & Baseline & 58.2  & 56.2  & 19.4   & 14.8  & 29.8  & 37.2 & 11.8 & 29.8   \\
                                   & Ours     & 70.8  & 77.8  & 28.8   & 30.4  & 42.4  & 49.4 & 25.6 & 46.8   \\
                                   & Random   & 67.2  & 73.0  & 26.6   & 24.2  & 38.2  & 47.8 & 22.6 & 43.4   \\
\bottomrule
\end{tabular}
\end{table*}

==> AAAI2022/tables/tab-voc.tex <==
\begin{table*}[]
\centering
\caption{White-box and black-box attack performance on different models with different perturbation budgets using PASCAL VOC dataset.}
\label{tab:voc}
\begin{tabular}{cccc|cccccc}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Perturbation \\ Budget\end{tabular}} &
  \multirow{2}{*}{Method} &
  \multicolumn{2}{c|}{\textbf{Whitebox}} &
  \multicolumn{6}{c}{\textbf{Blackbox}} \\ \cline{3-10} 
                                   &          & FRCNN & YOLOv3 & Retina & Libra & Fovea & Free & DETR & D-DETR \\ \hline
\multirow{3}{*}{$L_{\infty} = 5$}  & Baseline & 13.2  & 29.2   & 4.8    & 4.2   & 8.0   & 13.4 & 5.0  & 12.2   \\
                                   & Ours     & 24.8  & 50.0   & 8.8    & 9.0   & 16.6  & 21.4 & 11.2 & 25.6   \\
                                   & Random   & 20.0  & 46.2   & 8.4    & 7.4   & 15.0  & 20.0 & 8.8  & 20.2   \\ \hline
\multirow{3}{*}{$L_{\infty} = 10$} & Baseline & 40.0  & 53.8   & 13.8   & 9.2   & 22.2  & 27.4 & 9.6  & 23.2   \\
                                   & Ours     & 55.8  & 75.6   & 22.6   & 20.4  & 33.6  & 39.2 & 20.2 & 39.2   \\
                                   & Random   & 52.4  & 69.2   & 19.4   & 17.4  & 31.6  & 37.8 & 17.4 & 36.8   \\ \hline
\multirow{3}{*}{$L_{\infty} = 20$} & Baseline & 65.2  & 67.8   & 24.0   & 21.4  & 34.4  & 41.8 & 14.4 & 37.6   \\
                                   & Ours     & 78.6  & 87.2   & 35.2   & 38.4  & 51.6  & 56.6 & 34.0 & 58.4   \\
                                   & Random   & 74.4  & 83.8   & 31.0   & 29.6  & 46.2  & 54.4 & 28.0 & 52.6   \\ \hline
\multirow{3}{*}{$L_{\infty} = 30$} & Baseline & 70.6  & 70.4   & 29.8   & 28.6  & 41.6  & 48.0 & 20.4 & 38.6   \\
                                   & Ours     & 80.6  & 88.0   & 42.0   & 44.2  & 56.8  & 63.6 & 40.2 & 59.0   \\
                                   & Random   & 79.2  & 82.6   & 37.8   & 36.8  & 53.4  & 59.8 & 34.4 & 52.8   \\ \hline
\multirow{3}{*}{$L_{\infty} = 40$} & Baseline & 73.4  & 73.2   & 30.8   & 27.0  & 41.8  & 47.6 & 21.6 & 41.2   \\
                                   & Ours     & 85.4  & 90.2   & 43.6   & 45.2  & 60.2  & 63.4 & 41.8 & 62.4   \\
                                   & Random   & 82.2  & 85.4   & 40.0   & 38.8  & 54.0  & 62.2 & 37.0 & 57.4   \\ \hline
\end{tabular}
\end{table*}
